On Low-Risk Heavy Hitters and Sparse Recovery Schemes

We study the heavy hitters and related sparse recovery problems in the low-failure probability regime. This regime is not well-understood, and has only been studied for non-adaptive schemes. The main previous work is one on sparse recovery by Gilbert et al.(ICALP'13). We recognize an error in their analysis, improve their results, and contribute new non-adaptive and adaptive sparse recovery algorithms, as well as provide upper and lower bounds for the heavy hitters problem with low failure probability.

==> countsketch.tex <==
% !TeX root = main.tex

\section{$\ell_2$ Heavy hitters Upper Bound}


In this section we give our algorithm for $\ell_2$ heavy hitters under Guarantee $3$. Let $d = C_d \log(\epsilon n)$ and $B = C_B/\epsilon$, for constants $C_d,C_B$ to be chosen later. 
For $r \in [d]$ we pick hash functions $h_r: [n] \rightarrow [B]$, and also $n\times d$ independent standard gaussians, which we denote by $g_{i,r}$. We then perform measurements


	\[ \forall j \in [B], r \in [d] :	y_{j,r} = \sum_{ i \in h_r^{-1}(j)} g_{i,r} x_i.		\]



The total number of measurements/rows of the linear sketch equals $\Oh(\epsilon^{-1} \log(\epsilon n))$. The query algorithm operates in the following way: For every $i \in [n]$, it estimates

	\[	\hat{x}_i = \mathrm{median}_{r \in [d]}{ | y_{h_r(i),r} |},	\]


and keeps the largest $C_L k $ coordinates, forming list $L$. We now claim that $H_{1/\epsilon,1}(x) \subset L$. The following lemma is the main technical part of our argument. In what follows $c_T$ is an absolute constant.


\begin{lemma}

Let $T$ be a set of size $c_Tk$ such that $T \cap H_{1/(10\epsilon)}(x) = \emptyset$, and let $i^*$ be some element of $H_{1/\epsilon,\epsilon}(x)$. Then,


\[	\mathbb{P} \left[ \forall i \in T , \hat{x}_i > \hat{x}_{i^*} \right] \leq e^{-\Omega(1/\epsilon(\epsilon \log n))}	\]

\end{lemma}


\begin{proof}


%First of all, we define the vector $y^*$, which does not contain the contribution of coordinates $i \in T$. Namely, one can obtain $y^*$ from $y$ by the following set of operations


%	\[	\forall i \in T, \forall r \in [d]: y^*_{h_r(i),r)} \leftarrow y_{h_r(i),r)} - g_{i,h_r(i)}x_i.	\]

%Next, we define the following set of buckets/measurements.

%\[	B_r = \{ (j,r): |y^*_{j,r}| \geq \frac{\epsilon}{10k} \|x_{-1/\epsilon}\|_2.	\]


%We claim that $|B_r| = \Oh(k)$. 

Fix $r$ and observe that at $(1-\eta)|T|$ coordinates in $T$ will be isolated under $h_r$ with probability $e^{-\Omega(k)}$, by setting $C_B$ sufficiently large. Let this set of coordinates be $T_r'$. There exist at most $(C+1)/\epsilon$ indices $j \in [b]$ for which 
\[\sum_{i \in h^{-1}_r(j) \setminus T} x_i^2 \geq \frac{\epsilon}{C} \|x_{-1/\epsilon}\|_2,\] 

for some large enough constant $C$. Let the set of these buckets called $B_r$. For some small enough absolute constant $\zeta,$ we also have that


	\[	\mathbb{P} \left[ ||T_r'| \cap B_r| \geq |T|\zeta\cdot c_T/\epsilon\right] \leq { c_T/\epsilon \choose \zeta c_T /\epsilon } \left( \frac{c_T}{C_B} \right)^{\zeta c_T/\epsilon} = e^{-\Omega(1/\epsilon)},	\]


where the constant in the exponent can become arbitrarily large by tuning $C_B$ to be large enough.
This means that $|T_r' \setminus B_r| \geq (1-\zeta - \eta)|T| = (1-\eta')c_Tk$, with all but $e^{-\Omega(1/\epsilon)}$ failure probability. Observe that all $y_{h_r(i),r}$ follow a normal distribution, and with at most constant probability $|y_{h_r(i),r}|$ will drop below $1/2\|x_{i \in h_r^{-1}(j)}\|_2$, and also with at most constant probability will rise above $2\|x_{i \in h_r^{-1}(j)}\|_2$, by setting $C$ to be large enough we get


	\[	\mathbb{P} \left[ \exists S \subset T_r' \setminus B_r, |S| \geq \eta'|T|, \forall i \in S: |y_{h_r(i^*),r}| \leq |y_{h_r(i),r}|\right] \leq {c_T/\epsilon \choose \eta'c_T/\epsilon} ( \frac{1}{C'} )^{\eta'c_T/\epsilon} = e^{-\Omega(k)},		\]

for some constant $C'$ depending on $C$. Also, the constant inside the exponent of the failure probability can become arbitrarily large by tuning $C,C'$. 

Account for all diferent $d$ values of $r$, we get in at least $9d/10$ of the iterations $r$, $|y_{h_r(i^*),r)}|$ will be larger than $|y_{h_r(i),r}|$, for least $(1-\eta')|T|$ coordinates $i \in T$. This implies that the total number of pairs $(i,r)$ with $i \in T$, for which $|y_{h_r(i^*),r)}| > |y_{h_r(i),r}|$, is at least $9d/10 \cdot (1-\eta')|T|$. Now, if the $\hat{x}_{i^*} < \hat{x}_i$ for all $i \in T$, we would get that the total number of those pairs would be at most $d/2 \cdot |T| < 9d/10(1-\eta') |T|$, for $\eta'$ small enough. The above argument allows us to take a union bound over all $2/ \epsilon {n \choose \epsilon}$ pairs $(i^*,T)$ and complete the proof of the lemma.

\end{proof}


Having the above lemma, the argument proceeds exactly as in the case of \textsc{CountMin} sketch, by setting $c_L = c_T + c$.

